Deep Learning for Detecting Multiple Space-Time Action Tubes in Videos

In this work, we propose an approach to the spatiotemporal localisation (detection) and classification of multiple concurrent actions within temporally untrimmed videos. Our framework is composed of three stages. In stage 1, appearance and motion detection networks are employed to localise and score actions from colour images and optical flow. In stage 2, the appearance network detections are boosted by combining them with the motion detection scores, in proportion to their respective spatial overlap. In stage 3, sequences of detection boxes most likely to be associated with a single action instance, called action tubes, are constructed by solving two energy maximisation problems via dynamic programming. While in the first pass, action paths spanning the whole video are built by linking detection boxes over time using their class-specific scores and their spatial overlap, in the second pass, temporal trimming is performed by ensuring label consistency for all constituting detection boxes. We demonstrate the performance of our algorithm on the challenging UCF101, J-HMDB-21 and LIRIS-HARL datasets, achieving new state-of-the-art results across the board and significantly increasing detection speed at test time. We achieve a huge leap forward in action detection performance and report a 20% and 11% gain in mAP (mean average precision) on UCF-101 and J-HMDB-21 datasets respectively when compared to the state-of-the-art.

==> text/contrib.old.tex <==
\paragraph{Contributions}
In this paper we propose an algorithm for human action detection and segmentation in 
which configurations of region proposals in each frame are assigned a cost and the 
spatio-temporal action tubes are extracted via two passes of dynamic programming.
Moreover, by taking advantage of the human foreground-background segmentation work by \cite{Lu_2015_CVPR},
we generate action frame proposals based on the power set of 
\hlr{connected components} in the foreground-background segmentation.
This means that we can output a pixel-level action instance segmentation 
in addition to detection of tubes.
%We propose an `actionness' measure to prune region proposals as per their `actionness' scores.
%To this end, we demonstrated that human actions which exhibit very negligible bodily movements can also be detected based on our `actionness' measure.  
Although our method builds upon action tube work by Gkioxari and Malik \etal \cite{Georgia-2015a}, 
we extend action tube search to untrimed video with co-ocurring action and 
instance level segmentation of actions. 
To the best of our knowledge our algorithm provides the 
best human action detection results on the most challenging datasets available to date.
%We show spatio-temporal tube detection result on UCF101 and LIRIS Harl dataset.
Lastly, we are the first to show qualitative action instance segmentation results on LIRIS-HARL dataset.
%OUTLINE THE PIPELINE/METHODOLOGY HERE - ALSO PUT A DIAGRAM SIMILAR TO THAT OF GOOGLE
%ALSO MAKE CLEARER WHAT IS NOVEL IN EACH STEP
